STAFF: Stateful Taint-Assisted Full-system Firmware Fuzzing

Modern embedded Linux devices, such as routers, IP cameras, and IoT gateways, rely on complex software stacks where numerous daemons interact to provide services. Testing these devices is crucial from a security perspective since vendors often use custom closed- or open-source software without documenting releases and patches. Recent coverage-guided fuzzing solutions primarily test individual processes, ignoring deep dependencies between daemons and their persistent internal state. This article presents STAFF, a firmware fuzzing framework for discovering bugs in Linux-based firmware built around three key ideas: (a) user-driven multi-request recording, which monitors user interactions with emulated firmware to capture request sequences involving application-layer protocols (e.g., HTTP); (b) intra- and inter-process dependency detection, which uses whole-system taint analysis to track how input bytes influence user-space states, including files, sockets, and memory areas; (c) protocol-aware taint-guided fuzzing, which applies mutations to request sequences based on identified dependencies, exploiting multi-staged forkservers to efficiently checkpoint protocol states. When evaluating STAFF on 15 Linux-based firmware targets, it identifies 42 bugs involving multiple network requests and different firmware daemons, significantly outperforming existing state-of-the-art fuzzing solutions in both the number and reproducibility of discovered bugs.

==> sections/byte_annotation_complexity.tex <==

\paragraph{Computational Complexity.}
We analyze time and space using the following symbols:
\begin{itemize}
    \item \(R\) = \#regions in a seed; 
    \item \(N_r\) = length of region \(r\);
    \item \(D\) = total number of explicit region-to-region dependencies across all files;
    \item \(N_{\max}=\max_r N_r\); 
    \item \(M=\sum_{r=0}^{R-1}N_r\) (total bytes across regions);
    \item \(\ell\) = effective subsequence length bound when the trie \texttt{T} is successfully built (\(\ell\le \texttt{INITIAL\_MAX\_LEN\_CONST}\));
    \item \(E=\lvert s.\texttt{tainted\_memory\_events}\rvert\); 
    \item \(U=\) \#distinct PCs in the trace.
\end{itemize}
For an event window passed to \texttt{AnnotateSubregion}, let \(L\) denote the length of the longer of its load/store sequences. We assume average \(O(1)\) child lookup per trie step (hash map or fixed 256-way array).

\smallskip
\noindent\textbf{(1) Trie construction (\autoref{alg:byte-annotation-emilio} lines~\ref{line:init-maxlen}--\ref{line:insert-end}, \autoref{alg:trie-insert-emilio}).}
For a single region of length \(N_r\), \texttt{TrieInsert} considers every start index \(i\in[0,N_r-1]\) and extends up to 
\(\min(\ell,\,N_r-i)\) bytes (lines~\ref{line:trie-start}--\ref{line:trie-byte-loop}). 
Hence the number of node-steps is
\[
\sum_{i=0}^{N_r-1}\min(\ell,\,N_r-i)
\]

Analyzing this expression, we can identify two cases.
\begin{itemize}
    \item \textbf{Case 1: \(N_r \ge \ell\).} The sum evaluates to 
    \(N_r\ell - \frac{\ell(\ell-1)}{2}\). Here, \(N_r\ell\) dominates \(\frac{\ell(\ell-1)}{2}\) asymptotically, so the total node-steps are \(\Theta(N_r\ell)\).
    
    \item \textbf{Case 2: \(N_r < \ell\).} The sum evaluates to \(\frac{N_r(N_r+1)}{2}\), which is a triangular number and grows like \(\Theta(N_r^2)\). Here the maximum subsequence length \(\ell\) does not constrain the sum because \(N_r < \ell\).
\end{itemize}

Combining both cases gives
\[
\sum_{i=0}^{N_r-1}\min(\ell,\,N_r-i)
=
\begin{cases}
N_r\ell - \frac{\ell(\ell-1)}{2}, & N_r\ge \ell,\\[2mm]
\frac{N_r(N_r+1)}{2}, & N_r<\ell.
\end{cases}
\]
since:
\begin{itemize}
    \item if \(N_r \ge \ell\), \(\min\{N_r\ell, N_r^2\} = N_r\ell\) (matches Case 1),
    \item if \(N_r < \ell\), \(\min\{N_r\ell, N_r^2\} = N_r^2\) (matches Case 2).
\end{itemize}

\noindent Each node-step performs an existence check/creation, a pointer move, and one metadata append, all \(O(1)\) on average. Therefore, per region:
\[
T_r = \Theta(\min\{N_r\ell,\,N_r^2\}),
\]
and across all regions:
\[
T_{\text{trie}} = \sum_r T_r = \Theta\!\Big(\sum_r \min\{N_r\ell,\,N_r^2\}\Big) \subseteq O(M\ell).
\]

\smallskip
\noindent\textbf{(2) Initialization of \texttt{annotated\_bytes} (\autoref{alg:byte-annotation-emilio} \ref{line:init-ann-start}--\ref{line:init-ann-end}).}
We allocate one record per input byte and initialize two empty sets per record leading to a cost of \(\Theta(M)\).

\smallskip
\noindent\textbf{(3) Event windowing (\autoref{alg:process-mem-events-emilio}).}
Each call starts with an \(O(1)\) PC dedup check (\ref{line:pc-check}). 
If the PC is new, we extend a contiguous window while region and GPA remain aligned (\ref{line:for-events}--\ref{line:window-break}); this costs \(O(W)\) where \(W\) is the length of that contiguous block. Because subsequent events with already-seen PCs return immediately, each PC contributes the window-building cost at most once. Summed over all distinct PCs, window building is \(O(E)\). The call then forwards one window to \texttt{AnnotateSubregion}.

\smallskip
\noindent\textbf{(4) Subregion annotation (\autoref{alg:annotate-subregion-emilio}).}
Let \(L\) be the length of the longer of the two sequences \(\texttt{E[type]}\) (for \(type\in\{\texttt{load},\texttt{store}\}\)). 
We set the minimum candidate length \(\texttt{minL}\) (line~\ref{line:min-subregion}), then enumerate all subsequences from length \(L\) down to \(\texttt{minL}\) (lines~\ref{line:for-len}--\ref{line:for-k}). 

We calculate the number of candidated subsequences \#\text{cands} of \(L\). Let the windowed sequence have length $L$, and consider subsequences of length $s$. For length $s$, the number of possible starting positions is: $L - s + 1$.
because the first element can start at positions $1,2,\dots,L-s+1$. We enumerate subsequences from length $\texttt{minL}$ up to $L$, giving
\[
\#\text{cands} = \sum_{s=\texttt{minL}}^L (L - s + 1) = 1 + 2 + \dots + (L - \texttt{minL} + 1).
\]
Applying the arithmetic series formula where the sum of the first $n$ integers is $1 + 2 + \dots + n = \frac{n(n+1)}{2}$, we have
\[
\#\text{cands} = \frac{(L - \texttt{minL} + 1)(L - \texttt{minL} + 2)}{2} = \Theta\big((L - \texttt{minL} + 1)^2\big).
\]
And since $L - \texttt{minL} + 1 \le L$, we have
\[
\#\text{cands} = O(L^2).
\]
On a successful unique match, we have
\[
\#\text{cands} = 1.
\]
A trie lookup for the longest subsequence of length \(L\) takes \(\Theta(L)\) time (one step per byte). 
Hence, the total lookup cost is:
\[
\#\text{cands} \cdot \Theta(L)
\]
Thus, taking in consideration $L$, the \emph{best-case} cost per window is \(\Theta(L)\) if the first candidate matches uniquely.
In the \emph{worst-case}, the cost per window is \(O(L^3)\).

Raising \(\texttt{minL}\) prunes short subsequences, reducing the number of candidates and the total lookup cost, without changing asymptotic worst-case \(O(L^3)\), but lowering constants.

\smallskip
\noindent\textbf{(5) Region dependencies filtering (\autoref{alg:filter-region-deps}, \autoref{alg:build-filtered-deps-map}).}  
Region dependency filtering involves three main steps. First, constructing the \texttt{fmd} map (line~\ref{line:fmd-init}) requires iterating over the entries of the \texttt{s.region\_deps} map (lines~\ref{line:fmd-foreach-dst}--\ref{line:fmd-foreach-dst-end}), which costs \(O(D)\). Second, organizing the \texttt{nodes} and \texttt{dep\_edges} maps (lines~\ref{line:nodes-init}--\ref{line:add-node-file}) also iterates over all map entries, again costing \(O(D)\). Finally, the recursive \texttt{BuildFilteredDeps()} function traverses the directed acyclic graph of region dependencies. In the worst case, every region may depend directly or indirectly on every other region, and each file may be associated with a dependency, so the total cost of propagating filtered assignments is bounded by \(O(D R)\). Thus, the overall computational cost of region dependency filtering is 
\[
O(D) + O(D) + O(D R) = O(D R).
\]

\smallskip
\noindent\textbf{(6) Overall per-seed computational bounds.}
Combining trie construction, subregion annotation, and region dependency filtering:

\[
\begin{aligned}
T_{\text{seed}} &= O(M\ell) \;\; (\text{trie, Alg.~\ref{alg:trie-insert-emilio}}) \\
&\;+ \sum_{\text{windows}} O(L^3) \;\; (\text{annotated bytes, Alg.~\ref{alg:byte-annotation-emilio}}) \\
&\;+ O(D R) \;\; (\text{region deps filtering, Algs.~\ref{alg:filter-region-deps}-\ref{alg:build-filtered-deps-map}}) \\
&= O(M\ell) + \sum_{\text{windows}} O(L^3) + O(D R)
\end{aligned}
\]

\paragraph{Spatial Complexity.}
We analyze memory usage using the same symbols as above, explicitly referring to the algorithms and pseudocode lines where each structure is allocated.

\smallskip
\noindent\textbf{(1) Trie storage (\texttt{T}).}  
Each inserted subsequence creates a chain of trie nodes 
(\autoref{alg:trie-insert-emilio}, lines~\ref{line:trie-move-node}--\ref{line:trie-append-pos}).  
Let $n_r$ be the number of node-steps for region $r$, as computed in the time analysis:
\[
n_r = \sum_{i=0}^{N_r-1} \min(\ell, N_r-i) 
= \Theta(\min\{N_r \ell, N_r^2\}).
\] 
Each trie node stores:
\begin{itemize}
    \item a reference to its children (hash/dict entry),
    \item a dynamic list \texttt{positions}, where each element is a pair 
    $(\texttt{position}, \texttt{region\_id})$ 
    (\ref{line:trie-append-pos}).
\end{itemize}
Thus, memory per node is $O(1)$ on average. Summed over all regions:
\[
S_{\text{trie}} = \sum_r O(n_r) = O\!\Big(\sum_r \min\{N_r\ell, N_r^2\}\Big) \subseteq O(M \ell).
\]

\smallskip
\noindent\textbf{(2) Annotated bytes array.}  
In \autoref{alg:byte-annotation-emilio}, lines~\ref{line:init-ann-start}--\ref{line:init-ann-end}, 
we allocate one record per input byte.  
Each record contains two initially empty sets \texttt{deps} and \texttt{PCs}, which grow during subregion annotation. Hence:
\[
S_{\text{annotated\_bytes}} = O(M).
\]

\smallskip
\noindent\textbf{(3) Event windows and candidate subsequences.}  
In \autoref{alg:process-mem-events-emilio}, the loop 
(\ref{line:for-events}--\ref{line:window-break}) extends contiguous blocks of memory events into a window, which is then forwarded to 
\texttt{AnnotateSubregion}.  
Within \autoref{alg:annotate-subregion-emilio}, we copy the window of length $L$ into local load/store buffers 
(\ref{line:for-len}--\ref{line:for-k}). Before being annotated, two buffers (one for store and one for load) are retained. At most two candidate subsequences of length $L$ resides in memory at a time. Thus the per-window buffer usage is
\[
O(2L)
\]

\smallskip
\noindent\textbf{(4) Region dependencies filtering (\autoref{alg:filter-region-deps}, \autoref{alg:build-filtered-deps-map}).}  
The main data structures used are the \texttt{fmd} map, the \texttt{nodes} map, and the \texttt{dep\_edges} map. Each of these structures stores information proportional to the number of file-based dependencies \(D\) and the number of regions \(R\):
\begin{itemize}
    \item \texttt{fmd} map: stores, for each destination region, the files contributing to dependencies, costing \(O(D)\) space.
    \item \texttt{nodes} map: stores one entry per region and file combination, costing \(O(D)\) space.
    \item \texttt{dep\_edges} map: stores adjacency lists for the DAG of region dependencies, costing \(O(D)\) space.
\end{itemize}
Overall, the spatial complexity is dominated by storing the filtered assignments and dependency edges, yielding
\[
S_{\text{region-deps}} = O(D + D + D) = O(D).
\]

\smallskip
\noindent\textbf{(5) Overall per-seed spatial bound.}  
Combining the above contributions:

\[
\begin{aligned}
S_{\text{seed}} &= O(M\ell) && \text{(trie, Alg.~\ref{alg:trie-insert-emilio})} \\
&\;+ O(M) && \text{(annotated bytes, Alg.~\ref{alg:byte-annotation-emilio})} \\
&\;+ O(L_{\max}) && \text{(windows and candidates, 
Algs.~\ref{alg:process-mem-events-emilio},~\ref{alg:annotate-subregion-emilio})} \\
&\;+ O(D) && \text{(region deps filtering, Algs.~\ref{alg:filter-region-deps},~\ref{alg:build-filtered-deps-map})}.
\end{aligned}
\]

Since \(O(M \ell)\) dominates for nontrivial \(\ell\), the asymptotic spatial complexity per seed remains

\[
S_{\text{seed}} = O(M \ell).
\]

==> sections/taint_hints_complexity.tex <==
\paragraph{Computational Complexity.} 
Let us define the following symbols:

\begin{itemize}
    \item $S$ = the set of seeds;
    \item $R$ = the maximum number of regions per seed;
    \item $L$ = the maximum number of byte annotations per region;
    \item $P$ = the maximum number of program counters (PCs) per byte annotation.
\end{itemize}

\begin{enumerate}
    \item For each seed $s \in S$ \text{(line~\ref{line:for-seed})}, the algorithm iterates over all regions of $s$ (at most $R$ regions per seed) \text{(line~\ref{line:for-i})}.  
    For each region, it iterates over all byte annotations (at most $L$ per region) \text{(line~\ref{line:for-j})}.  
    For each byte, it first iterates over each \emph{active PC} (at most $P$) \text{(line~\ref{line:for-found-PCs})} and then, separately, over all PCs associated with that byte \text{(line~\ref{line:for-PCs})}.
    
    \item For each seed $s \in S$ \text{(line~\ref{line:for-j})}, the algorithm iterates again over all its regions (at most $R$ per seed) \text{(line~\ref{line:for-i})}.  
    For each region, it processes all region dependencies \text{(line~\ref{line:for-region})}.  
    Let the maximum number of dependencies per region be denoted by $D$.

    \item For each seed $s \in S$ \text{(line~\ref{line:for-seed})}, the algorithm iterates over all regions (at most $R$ per seed) \text{(line~\ref{line:for-i})}.  
    For each region, it iterates once more over all \emph{active PCs} \text{(line~\ref{line:final-for-found-PCs})}.
\end{enumerate}

Hence, the total number of iterations for processing all PCs across all byte annotations and regions is at most
\[
|S| \cdot R \cdot L \cdot P.
\]

Additionally, for each region, the algorithm performs sorting and filtering of hints.  
Let $|H[s]_i|$ denote the number of hints in the $i$-th region of seed $s$. Sorting and filtering each region costs
\[
O(|H[s]_i| \log |H[s]_i|).
\]

Summing over all regions of all seeds, the total cost for sorting and filtering hints is
\[
\begin{aligned}
S_{\text{hints}} &= \sum_{s \in S} \sum_{i=1}^{R} O(|H[s]_i| \log |H[s]_i|) \\
&= O\!\left( \sum_{s \in S} \sum_{i=1}^{R} |H[s]_i| \log |H[s]_i| \right) \\
&= O\!\left( |S| \cdot \sum_{i=1}^{R} |H[s]_i| \log |H[s]_i| \right).
\end{aligned}
\]

Combining both contributions, the worst-case time complexity of the algorithm is
\[
T_{\text{taint\_hints}} = O\!\left( |S| \cdot R \cdot L \cdot P \;+\; |S| \cdot \sum_{i=1}^{R} |H[s]_i| \log |H[s]_i| \right).
\]

\noindent Here, the first term accounts for iterating over all byte annotations and PCs (lines~\ref{line:for-i}--\ref{line:final-for-found-PCs-end}), while the second term accounts for sorting and filtering hints per region (line~\ref{line:filter-hints-call}). We assume that per-PC operations (such as unions of dependency sets) are constant-time, as the number of dependencies per PC is bounded.

\paragraph{Spatial Complexity.}
Let us analyze the memory requirements of the algorithm.  
We use the same symbols $S$, $R$, $L$, $P$, and $D$ as above.

\begin{enumerate}
    \item For each seed $s \in S$ \text{(line~\ref{line:for-seed})}, the algorithm stores all its regions (at most $R$ per seed) \text{(line~\ref{line:for-i})}.  
    For each region, it stores all byte annotations (at most $L$ per region) \text{(line~\ref{line:for-j})}, and for each byte annotation, the set of associated PCs (at most $P$) \text{(line~\ref{line:for-PCs})}.  
    Hence, the storage required for byte--PC associations is bounded by
    \[
    O(|S| \cdot R \cdot L \cdot P).
    \]

    \item For each region, the algorithm also stores the set of region dependencies (at most $D$ per region) \text{(line~\ref{line:for-region})}.  
    Hence, the space required for dependencies is
    \[
    O(|S| \cdot R \cdot D).
    \]

    \item Additionally, each region may contain a set of hints $H[s]_i$, which must be stored before sorting and filtering \text{(line~\ref{line:filter-hints-call})}.  
    Thus, the space needed for hints across all regions and seeds is
    \[
    O\!\left( \sum_{s \in S} \sum_{i=1}^{R} |H[s]_i| \right).
    \]
\end{enumerate}

Combining all contributions, the total spatial complexity of the algorithm is

\[
\begin{aligned}
S_{\text{taint\_hints}} &= O\!\left(|S|RL P \;+\; |S|RD \;+\; \sum_{s \in S}\sum_{i=1}^R |H[s]_i|\right) \\
&= O\!\left(|S|RL P \;+\; |S|RD \;+\; |S|\sum_{i=1}^R |H[s]_i|\right).
\end{aligned}
\]


\noindent Here, the first term accounts for storing per-byte PC associations (lines~\ref{line:for-i}--\ref{line:for-PCs}), the second for region dependencies (line~\ref{line:for-region}), and the third for per-region hints (line~\ref{line:filter-hints-call}).
